Decentralised Resource Allocation and Coordination for 5G Cellular Communication Networks

In order to cope with the ever increasing traffic load that networks will need to support, a new approach for planning cellular networks deployments should be followed. Traditionally, cell association and resource allocation has been based on the received signal power but this approach seems to be inadequate regarding the brewing of heterogeneous networks. In this work, we first implement a network simulator in order to test new cell associacion and resource allocation techniques. Then, we pose the network utility maximisation problem, reformulating the Downlink and Uplink Decoupling (DUDe) scheme under the framework and tools of mathematical optimisation. We derive the explicit solution of the problem under fixed and non-fixed association policy so as to propose and develope both centralised and decentralised algorithms capable of solving cell association and resource allocation problems. We observe that the decentralised approach requires low computational effort and represents a significant gain in the overall performance of the network.

==> custom_settings.tex <==
% -*- TeX Mode -*-
%
%   Use this file for your own custom packages, command-definitions, etc...
%

\usepackage{multirow}
\usepackage{footnote}
\usepackage{amsmath}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{amsthm}
\newtheorem{remark}{Remark}[chapter]
\usepackage[outdir=./]{epstopdf}
\newcommand{\norm}[1]{\lVert#1\rVert}

